Direct measurements of carbon and sulfur isotope ratios in the Milky Way

With the IRAM 30 meter telescope, we performed observations of the $J$ = 2-1 transitions of CS, C$^{33}$S, C$^{34}$S, C$^{36}$S, $^{13}$CS, $^{13}$C$^{33}$S, and $^{13}$C$^{34}$S as well as the $J$ = 3-2 transitions of C$^{33}$S, C$^{34}$S, C$^{36}$S, and $^{13}$CS toward a large sample of 110 HMSFRs. We measured the $^{12}$C/$^{13}$C, $^{32}$S/$^{34}$S, $^{32}$S/$^{33}$S, $^{32}$S/$^{36}$S, $^{34}$S/$^{33}$S, $^{34}$S/$^{36}$S, and $^{33}$S/$^{36}$S abundance ratios with rare isotopologs of CS, thus avoiding significant saturation effects. With accurate distances obtained from parallax data, we confirm previously identified $^{12}$C/$^{13}$C and $^{32}$S/$^{34}$S gradients as a function of galactocentric distance (RGC). In the CMZ, $^{12}$C/$^{13}$C ratios are higher than suggested by a linear fit to the disk values as a function of RGC. While $^{32}$S/$^{34}$S ratios near the Galactic center and in the inner disk are similar, this is not the case for $^{12}$C/$^{13}$C, when comparing central values with those near RGC of 5 kpc. As was already known, there is no $^{34}$S/$^{33}$S gradient but the average ratio of 4.35~$\pm$~0.44 derived from the $J$ = 2-1 transition lines of C$^{34}$S and C$^{33}$S is well below previously reported values. A comparison between solar and local interstellar $^{32}$S/$^{34}$S and $^{34}$S/$^{33}$S ratios suggests that the Solar System may have been formed from gas with a particularly high $^{34}$S abundance. For the first time, we report positive gradients of $^{32}$S/$^{33}$S, $^{34}$S/$^{36}$S, $^{33}$S/$^{36}$S, and $^{32}{\rm S}/^{36}{\rm S}$ in our Galaxy. The predicted $^{12}$C/$^{13}$C ratios from the latest GCE models are in good agreement with our results. While $^{32}$S/$^{34}$S and $^{32}$S/$^{36}$S ratios show larger differences at larger RGC, $^{32}$S/$^{33}$S ratios show an offset across the entire inner 12 kpc of the Milky Way.

==> newTables/1allc36s_Table-corrected.tex <==
\begin{table*}[h]
\centering
\caption{\label{table_all36s}Isotope ratios of $^{34}$S/$^{36}$S and $^{32}$S/$^{36}$S}
\begin{tabular}{lc|cc|cc}
\hline\hline
Source  &   $R_{\rm GC}$   &  \multicolumn{2}{c}{$^{34}$S/$^{36}$S}   &  \multicolumn{2}{c}{$^{32}$S/$^{36}$S}    \\
        &    (kpc)           &    $J$ = 2-1    &   $J$ = 3-2          &    $J$ = 2-1    &   $J$ = 3-2            \\
\hline
W3OH            & 9.64 $\pm$ 0.03   &  140 $\pm$ 16  &  174 $\pm$ 29\tablefootmark{*}                   &  4181 $\pm$ 531  &  5195 $\pm$ 919\tablefootmark{*} \\
Orion-KL        & 8.54 $\pm$ 0.00   &  92  $\pm$ 53\tablefootmark{*}  &  83  $\pm$ 7                    &  1954 $\pm$ 1207\tablefootmark{*}  &  1765 $\pm$ 414  \\
$+$20 km~s$^{-1}$ cloud         & 0.03 $\pm$ 0.03   &  69  $\pm$ 11\tablefootmark{*}   &        $\cdots$                       &  1015 $\pm$ 278\tablefootmark{*}   &        $\cdots$     \\
$+$50 km~s$^{-1}$ cloud     & 0.02 $\pm$ 0.04   &  41  $\pm$ 4   &        $\cdots$                                        &  884 $\pm$ 104   &        $\cdots$     \\
G024.78$+$00.08 & 3.51 $\pm$ 0.15   &  151 $\pm$ 39\tablefootmark{*}  &  226 $\pm$ 66\tablefootmark{*}  &  2424 $\pm$ 699\tablefootmark{*}  &  3640 $\pm$ 1164\tablefootmark{*} \\
G030.81$-$00.05 & 5.73 $\pm$ 0.24   &  55  $\pm$ 15\tablefootmark{*}  &       $\cdots$                        &  829 $\pm$ 233\tablefootmark{*}  &       $\cdots$      \\
W51-IRS2        & 6.22 $\pm$ 0.06   &  109 $\pm$ 27\tablefootmark{*}  &  203 $\pm$ 45\tablefootmark{*}  &  1814 $\pm$ 506\tablefootmark{*}  &  3397 $\pm$ 855\tablefootmark{*} \\
DR21            & 8.10  $\pm$ 0.00   &  117 $\pm$ 24  &  159 $\pm$ 64\tablefootmark{*}                  &  3223 $\pm$ 742  &  4384 $\pm$ 1829\tablefootmark{*} \\
NGC7538         & 9.47 $\pm$ 0.07   &       $\cdots$       &  109 $\pm$ 28\tablefootmark{*}                   &       $\cdots$       &  2912 $\pm$ 897\tablefootmark{*} \\
\hline
\multicolumn{6}{c}{Below are the isotope ratios of $^{34}$S/$^{36}$S and $^{32}$S/$^{36}$S from \citet{1996A&A...313L...1M}} \\
\hline
W3OH                         & 9.64 $\pm$ 0.03   &   $\cdots$       &  181 $\pm$ 49  &  $\cdots$       &  4118 $\pm$ 1124  \\
Orion-KL                     & 8.54 $\pm$ 0.00   &   $\cdots$       &  104 $\pm$ 7   &  $\cdots$       &  2281 $\pm$ 174 \\
IRAS15491\tablefootmark{**}  & 5.48 $\pm$ 0.31   &   $\cdots$       &  108 $\pm$ 15  &  $\cdots$       &  2120 $\pm$ 307 \\
IRAS15520\tablefootmark{**}  & 5.67 $\pm$ 0.31   &   128 $\pm$ 32   &  133 $\pm$ 11  & 2531 $\pm$ 641  &  2629 $\pm$ 243 \\
IRAS16172\tablefootmark{**}  & 5.03 $\pm$ 0.29   &   121 $\pm$ 18   &  119 $\pm$ 14  & 2334 $\pm$ 361  &  2296 $\pm$ 287 \\
NGC6334A                     & 6.87 $\pm$ 0.12   &   108 $\pm$ 15   &  154 $\pm$ 20  & 2232 $\pm$ 322  &  3183 $\pm$ 431 \\
NGC6334B                     & 6.87 $\pm$ 0.12   &   163 $\pm$ 46   &  156 $\pm$ 26  & 3369 $\pm$ 960  &  3225 $\pm$ 552 \\
W51(M)                       & 6.22 $\pm$ 0.004  &   105 $\pm$ 11   &  104 $\pm$ 15  & 2119 $\pm$ 237  &  2099 $\pm$ 313 \\
\hline
\end{tabular}
\tablefoot{\tablefoottext{*}{Values with large uncertainties are derived from the tentive detection of C$^{36}$S lines.} \tablefoottext{**}{For these three sources without parallax data, their kinematic distances were estimated (for details, see Section~\ref{section_distance}).} The $^{34}$S/$^{36}$S and $^{32}$S/$^{36}$S isotope ratios in this work from the $J$ = 2-1 transition are corrected for the optical depth effects, while the ones for the 3-2 line could not be corrected.}
\end{table*}

==> newTables/1allratios.tex <==
\begin{table*}[h]
\caption{Interstellar C, N, O, S isotope ratios.}
\centering
\begin{tabular}{ccccccc}
\hline\hline
  & Molecule & CMZ & Inner disk &Local ISM & Outer Galaxy & Solar system\tablefootmark{*} \\
\hline
\label{table_allratios}
$^{12}$C/$^{13}$C & C$^{34}$S\tablefootmark{a}&  27 $\pm$ 3     &   41 $\pm$ 9  &   66 $\pm$ 10  &   74 $\pm$ 8   & 89     \\ 
          &        CN\tablefootmark{b}        & $\cdots$        &  44 $\pm$ 12  &   41 $\pm$ 11  &   66 $\pm$ 19  &      \\ 
          &      C$^{18}$O\tablefootmark{c}   &  24 $\pm$ 1     &   41 $\pm$ 2  &   60 $\pm$ 5   &   70 $\pm$ 10  &      \\ 
          &      H$_2$CO\tablefootmark{d}     & $\cdots$        &   40 $\pm$ 7  &   50 $\pm$ 13  &   64 $\pm$ 10  &      \\ 
          &            average                &   25 $\pm$ 2    &   42 $\pm$ 9  &   54 $\pm$ 10  &   69 $\pm$ 12  &       \\
\hline
$^{14}$N/$^{15}$N  & CN\tablefootmark{e}      & $\cdots$        &   269 $\pm$ 59   &   314 $\pm$ 104  &   289 $\pm$ 85  &  270 \\ 
          &   HCN\tablefootmark{f}            & $\cdots$        &    284 $\pm$ 63  &   398 $\pm$ 48   &   388 $\pm$ 32  &      \\ 
          &   HNC\tablefootmark{f}            & $\cdots$        &   363 $\pm$ 100  &   378 $\pm$ 79   &   395 $\pm$ 74  &      \\ 
          &    N$_2$H$^{+}$\tablefootmark{g}  & $\cdots$        &   900 $\pm$ 250  &   496 $\pm$ 65   &   581 $\pm$ 140 &      \\ 
          &   NH$_3$\tablefootmark{h}         &  40 $\pm$ 13    &   175 $\pm$ 46   &   297 $\pm$ 99   &   96 $\pm$ 44   &      \\
\hline
$^{16}$O/$^{18}$O & H$_2$CO\tablefootmark{i}  &   263 $\pm$ 45  &  327 $\pm$ 32    &  560 $\pm$ 25    &  625 $\pm$ 144  &  490 \\
$^{18}$O/$^{17}$O & CO\tablefootmark{j}       &  3.4 $\pm$ 0.1  &   3.6 $\pm$ 0.2  &   3.9 $\pm$ 0.4  &   4.8 $\pm$ 0.6 &  5.5 \\
$^{16}$O/$^{17}$O\tablefootmark{**}  &        &  894 $\pm$ 155  &  1177 $\pm$ 132  &  2184 $\pm$ 244  & 3000 $\pm$ 786  &  2625 \\
\hline
$^{32}$S/$^{34}$S\tablefootmark{a}  &         &  19 $\pm$ 2     &   18 $\pm$ 4      &   24 $\pm$ 4     &   28 $\pm$ 3     & 23   \\
$^{34}$S/$^{33}$S\tablefootmark{a}  &         &  4.2 $\pm$ 0.2  &   4.3 $\pm$ 0.4   &   4.2 $\pm$ 0.5  &   4.1 $\pm$ 0.3  & 5.6  \\
$^{32}$S/$^{33}$S\tablefootmark{a}  &         &   70 $\pm$ 16   &   82 $\pm$ 19     &   88 $\pm$ 21    &   105 $\pm$ 19   & 127  \\
$^{34}$S/$^{36}$S\tablefootmark{a}  &         &  41 $\pm$ 4     &   122 $\pm$ 18    &   111 $\pm$ 16   &   161 $\pm$ 32   & 200  \\
$^{32}$S/$^{36}$S\tablefootmark{a}  &         &  884 $\pm$ 104  &   2382 $\pm$ 368  &   2752 $\pm$ 458 &   4150 $\pm$ 828 & 4525 \\
\hline
\end{tabular}
\tablefoot{The inner disk values refer to the mean values at galactocentric distances of 2.0 kpc~$\le R_{\rm GC} \le$~6.0 kpc. The local ISM values refer to 7.5 kpc~$\le R_{\rm GC} \le$~8.5 kpc. The outer Galaxy values point to 9.0 kpc~$\le R_{\rm GC} \le$~11.0 kpc. 
\tablefoottext{*}{From \citet{1989GeCoA..53..197A}.} 
\tablefoottext{a}{This work.}
\tablefoottext{b}{From \citet{2002ApJ...578..211S} and \citet{2005ApJ...634.1126M}.}
\tablefoottext{c}{From \citet{1990ApJ...357..477L,1993ApJ...408..539L}, \citet{1996A&AS..119..439W}, and \citet{1998ApJ...494L.107K}.}
\tablefoottext{d}{From \citet{1980A&A....82...41H,1982A&A...109..344H,1983A&A...127..388H,1985A&A...143..148H} and \citet{2019ApJ...877..154Y}.}  
\tablefoottext{e}{From \citet{2012ApJ...744..194A}, \citet{2015ApJ...804L...3R}, and \citet{2015ApJ...808L..46F}. }  
\tablefoottext{f}{From \citet{2012ApJ...744..194A} and \citet{2018A&A...609A.129C}}  
\tablefoottext{g}{From \citet{2015ApJ...804L...3R}. }  
\tablefoottext{h}{From \citet{2021ApJS..257...39C}. }  
\tablefoottext{i}{From \citet{1981MNRAS.194P..37G} and \citet{1994ARA&A..32..191W}. }  
\tablefoottext{j}{From \citet{2020ApJS..249....6Z}. } 
\tablefoottext{**}{The $^{16}$O/$^{17}$O ratios are derived with values of $^{16}$O/$^{18}$O and $^{18}$O/$^{17}$O.}    }
\end{table*}

==> newTables/1allratiosCom.tex <==
\begin{table*}[h]
\caption{Comparison of isotope ratios at different galactocentric distances. Given are enhancements in percent.}
\centering
\begin{tabular}{ccccc}
\hline\hline
   & CMZ          &     CMZ      & Inner disk   &  Local ISM  \\
   & $\downarrow$ & $\downarrow$ & $\downarrow$ & $\downarrow$ \\
   &  Inner disk  & Outer Galaxy & Outer Galaxy & Solar system \\
\hline
\label{table_allratios_com}
$^{12}$C/$^{13}$C & 68 $\pm$ 33  &  176 $\pm$ 54  &  64 $\pm$ 21  &  65 $\pm$ 31  \\
\hline
$^{16}$O/$^{18}$O  & 24 $\pm$ 9  &  138 $\pm$ 61  &  91 $\pm$ 43   &  -12 $\pm$ 5   \\
$^{16}$O/$^{17}$O  & 32 $\pm$ 8  &  236 $\pm$ 111  &  155 $\pm$ 73  &  20 $\pm$ 13    \\
\hline
$^{32}$S/$^{34}$S  & -5 $\pm$ 11  &  47 $\pm$ 10  &  56 $\pm$ 18  &  -4 $\pm$ 17   \\
$^{32}$S/$^{33}$S  & 17 $\pm$ 8   &  50 $\pm$ 16  &  28 $\pm$ 6  &  44 $\pm$ 34 \\
$^{32}$S/$^{36}$S  & 169 $\pm$ 50  &  369 $\pm$ 125  &  74 $\pm$ 31  &  64 $\pm$ 27   \\
\hline
\end{tabular}
%\tablefoot{All values here are in percent.}
\end{table*}

==> newTables/1ratios32s_34s_doubleisotopes.tex <==
\begin{center}
\small
\begin{longtable}{lcc|ccc|cc|cc}
\caption{\label{table_doubleisotope} $^{32}$S/$^{34}$S isotope ratios derived through the double isotope method with the $J$ = 2-1 and $J$ = 3-2 transitions of C$^{34}$S and $^{13}$CS.}\\
\hline\hline
Source &  $V_{\rm LSR}$ & $R_{\rm GC}$  &   \multicolumn{3}{c}{Optical depth $J$ = 2-1} &  \multicolumn{2}{c}{Corrections for} &  \multicolumn{2}{c}{$^{32}$S/$^{34}$S}  \\
  &                &         &     &           &           &  \multicolumn{2}{c}{optical depth} &      &    \\
  &  (km s$^{-1}$) & (kpc)   &  CS & C$^{34}$S & $^{13}$CS &  $f_1$  &  $f_2$ &  2-1 & 3-2 \\
\hline
\endfirsthead
\caption{continued.}\\
\hline\hline
Source &  $V_{\rm LSR}$ & $R_{\rm GC}$  &   \multicolumn{3}{c}{Optical depth $J$ = 2-1} &  \multicolumn{2}{c}{Corrections for} &  \multicolumn{2}{c}{$^{32}$S/$^{34}$S}  \\
  &                &         &     &           &           &  \multicolumn{2}{c}{optical depth} &      &    \\
  &  (km s$^{-1}$) & (kpc)   &  CS & C$^{34}$S & $^{13}$CS &  $f_1$  &  $f_2$ &  2-1 & 3-2 \\
\hline
\endhead
\hline
\endfoot
WB89-380                & -86.62 & 14.19 $\pm$ 0.92 & 3.111 $\pm$ 0.598  & 0.135 $\pm$ 0.137 & 0.035 $\pm$ 0.000 & 1.1 & 1.0 &  21.20 $\pm$ 4.01  & 24.98 $\pm$ 4.69  \\ 
WB89-391                & -85.93 & 14.28 $\pm$ 0.94 & 5.189 $\pm$ 0.996  & 0.223 $\pm$ 0.226 & 0.058 $\pm$ 0.001 & 1.1 & 1.0 &  24.39 $\pm$ 4.64  & 20.98 $\pm$ 4.04  \\ 
W3OH                    & -46.96 & 9.64  $\pm$ 0.03 & 8.520 $\pm$ 1.671  & 0.310 $\pm$ 0.003 & 0.128 $\pm$ 0.001 & 1.2 & 1.1 &  26.15 $\pm$ 4.87  & 31.42 $\pm$ 5.85  \\ 
Orion-KL                & 8.24   & 8.54  $\pm$ 0.00 & 6.035 $\pm$ 1.189  & 0.166 $\pm$ 0.002 & 0.096 $\pm$ 0.001 & 1.1 & 1.0 &  24.75 $\pm$ 5.24  & 25.41 $\pm$ 4.86  \\ 
PointC1                 & -64.18 & 1.46  $\pm$ 0.15 & 0.588 $\pm$ 0.128  & 0.037 $\pm$ 0.000 & 0.021 $\pm$ 0.000 & 1.0 & 1.0 &  19.40 $\pm$ 4.55  &     $\cdots$      \\ 
G359.13$+$00.03         & -2.03  & 2.12  $\pm$ 1.14 & 5.526 $\pm$ 1.188  & 0.420 $\pm$ 0.004 & 0.179 $\pm$ 0.002 & 1.2 & 1.1 &  14.34 $\pm$ 4.11  &     $\cdots$      \\ 
SgrC                    & -44.31 & 0.24  $\pm$ 0.07 & 0.538 $\pm$ 0.123  & 0.048 $\pm$ 0.000 & 0.025 $\pm$ 0.000 & 1.0 & 1.0 &  12.81 $\pm$ 2.95  &     $\cdots$      \\ 
SgrC                    & 70.06  & 0.15  $\pm$ 0.03 & 0.406 $\pm$ 0.094  & 0.031 $\pm$ 0.000 & 0.019 $\pm$ 0.000 & 1.0 & 1.0 &  14.87 $\pm$ 3.38  &     $\cdots$      \\ 
$+$20~km~s$^{-1}$~cloud & 6.80   & 0.03  $\pm$ 0.03 & 4.523 $\pm$ 1.030  & 0.293 $\pm$ 0.003 & 0.200 $\pm$ 0.002 & 1.2 & 1.1 &  14.65 $\pm$ 3.20  & 15.13 $\pm$ 3.31  \\ 
G359.61$-$00.24         & 19.33  & 5.51  $\pm$ 0.15 & 4.307 $\pm$ 0.874  & 0.219 $\pm$ 0.002 & 0.092 $\pm$ 0.001 & 1.1 & 1.0 &  18.75 $\pm$ 3.66  & 21.66 $\pm$ 4.20  \\ 
$+$50~km~s$^{-1}$~cloud & 46.78  & 0.02  $\pm$ 0.04 & 3.096 $\pm$ 0.717  & 0.203 $\pm$ 0.002 & 0.147 $\pm$ 0.001 & 1.1 & 1.1 &  14.46 $\pm$ 3.20  & 14.59 $\pm$ 3.23  \\ 
CloudD                  & 23.32  & 0.67  $\pm$ 0.17 & 0.641 $\pm$ 0.144  & 0.040 $\pm$ 0.000 & 0.026 $\pm$ 0.000 & 1.0 & 1.0 &  14.47 $\pm$ 3.16  &     $\cdots$      \\ 
G000.37$+$00.03         & 39.98  & 0.19  $\pm$ 2.88 & 5.508 $\pm$ 1.266  & 0.283 $\pm$ 0.003 & 0.254 $\pm$ 0.003 & 1.1 & 1.1 &  15.78 $\pm$ 4.38  &     $\cdots$      \\ 
G0.25                   & 10.68  & 0.76  $\pm$ 0.53 & 1.590 $\pm$ 0.352  & 0.102 $\pm$ 0.001 & 0.061 $\pm$ 0.001 & 1.1 & 1.0 &  14.52 $\pm$ 3.20  &     $\cdots$      \\ 
G0.25                   & 38.59  & 0.37  $\pm$ 0.04 & 1.269 $\pm$ 0.290  & 0.091 $\pm$ 0.001 & 0.057 $\pm$ 0.001 & 1.0 & 1.0 &  14.79 $\pm$ 3.43  & 15.72 $\pm$ 3.98  \\ 
G000.31$-$00.20         & 18.43  & 5.25  $\pm$ 0.36 & 2.876 $\pm$ 0.585  & 0.158 $\pm$ 0.002 & 0.063 $\pm$ 0.001 & 1.1 & 1.0 &  15.71 $\pm$ 3.47  & 15.97 $\pm$ 3.54  \\ 
SgrB2                   & 53.93  & 0.44  $\pm$ 0.70 & 3.404 $\pm$ 0.780  & 0.207 $\pm$ 0.002 & 0.154 $\pm$ 0.002 & 1.1 & 1.1 &  17.47 $\pm$ 3.83  & 17.83 $\pm$ 3.91  \\ 
SgrB2                   & 80.88  & 0.41  $\pm$ 0.02 & 1.318 $\pm$ 0.304  & 0.083 $\pm$ 0.001 & 0.062 $\pm$ 0.001 & 1.0 & 1.0 &  17.09 $\pm$ 3.78  & 16.40 $\pm$ 3.65  \\ 
G1.28$+$0.07            & 98.64  & 0.30  $\pm$ 0.03 & 0.991 $\pm$ 0.225  & 0.048 $\pm$ 0.000 & 0.043 $\pm$ 0.000 & 1.0 & 1.0 &  12.45 $\pm$ 2.92  &     $\cdots$      \\ 
G1.28$+$0.07            & 177.50 & 0.18  $\pm$ 0.00 & 0.817 $\pm$ 0.187  & 0.049 $\pm$ 0.000 & 0.037 $\pm$ 0.000 & 1.0 & 1.0 &  15.65 $\pm$ 3.66  &     $\cdots$      \\ 
SgrD                    & -15.20 & 2.93  $\pm$ 3.62 & 6.357 $\pm$ 1.342  & 0.422 $\pm$ 0.004 & 0.183 $\pm$ 0.002 & 1.2 & 1.1 &  14.41 $\pm$ 2.92  & 18.67 $\pm$ 3.79  \\ 
SgrD                    & 40.31  & 0.76  $\pm$ 0.18 & 1.060 $\pm$ 0.238  & 0.072 $\pm$ 0.001 & 0.043 $\pm$ 0.000 & 1.0 & 1.0 &  15.48 $\pm$ 3.42  & 13.16 $\pm$ 2.99  \\ 
SgrD                    & 63.37  & 0.45  $\pm$ 0.07 & 0.448 $\pm$ 0.102  & 0.024 $\pm$ 0.000 & 0.020 $\pm$ 0.000 & 1.0 & 1.0 &  15.62 $\pm$ 4.08  &     $\cdots$      \\ 
G001.00$-$00.23         & 0.97   & 2.94  $\pm$ 7.03 & 9.963 $\pm$ 2.102  & 0.486 $\pm$ 0.005 & 0.286 $\pm$ 0.003 & 1.3 & 1.2 &  13.02 $\pm$ 3.60  &     $\cdots$      \\ 
Clump2                  & 14.19  & 4.20  $\pm$ 1.65 & 2.093 $\pm$ 0.428  & 0.085 $\pm$ 0.001 & 0.048 $\pm$ 0.000 & 1.0 & 1.0 &  37.16 $\pm$ 7.62  &     $\cdots$      \\ 
Clump2                  & 80.82  & 1.06  $\pm$ 0.10 & 1.500 $\pm$ 0.331  & 0.084 $\pm$ 0.001 & 0.057 $\pm$ 0.001 & 1.0 & 1.0 &  19.46 $\pm$ 4.19  & 14.69 $\pm$ 3.70  \\ 
Clump2                  & 141.00 & 0.60  $\pm$ 0.03 & 1.982 $\pm$ 0.445  & 0.113 $\pm$ 0.001 & 0.082 $\pm$ 0.001 & 1.1 & 1.0 &  25.43 $\pm$ 5.70  &     $\cdots$      \\ 
PointD1                 & 117.60 & 1.24  $\pm$ 0.07 & 0.340 $\pm$ 0.075  & 0.026 $\pm$ 0.000 & 0.012 $\pm$ 0.000 & 1.0 & 1.0 &  14.02 $\pm$ 2.99  &     $\cdots$      \\ 
G006.79$-$00.25         & 20.88  & 4.75  $\pm$ 0.25 & 10.743 $\pm$ 2.200 & 0.529 $\pm$ 0.005 & 0.247 $\pm$ 0.002 & 1.3 & 1.1 &  18.09 $\pm$ 3.53  & 21.30 $\pm$ 4.16  \\ 
G007.47$+$00.05         & -14.58 & 12.35 $\pm$ 2.49 & 4.106 $\pm$ 0.794  & 0.146 $\pm$ 0.001 & 0.052 $\pm$ 0.001 & 1.1 & 1.0 &  26.53 $\pm$ 5.92  & 29.52 $\pm$ 6.31  \\ 
G010.32$-$00.15         & 12.00  & 5.34  $\pm$ 0.29 & 5.185 $\pm$ 1.054  & 0.252 $\pm$ 0.003 & 0.112 $\pm$ 0.001 & 1.1 & 1.1 &  19.19 $\pm$ 3.73  & 21.62 $\pm$ 4.20  \\ 
G010.62$-$00.33         & -3.68  & 5.49  $\pm$ 0.56 & 2.809 $\pm$ 0.570  & 0.170 $\pm$ 0.002 & 0.060 $\pm$ 0.001 & 1.1 & 1.0 &  15.67 $\pm$ 3.52  & 18.19 $\pm$ 4.57  \\ 
G011.10$-$00.11         & 29.91  & 4.26  $\pm$ 0.21 &     $\cdots$       &    $\cdots$       &    $\cdots$       & $\cdots$ & $\cdots$ & $\cdots$ & 19.39 $\pm$ 5.60  \\ 
G013.71$-$00.08         & 46.81  & 4.59  $\pm$ 0.18 &     $\cdots$       &    $\cdots$       &    $\cdots$       & $\cdots$ & $\cdots$ & $\cdots$ & 17.28 $\pm$ 4.84  \\ 
G015.66$-$00.49         & -5.54  & 3.99  $\pm$ 0.50 & 2.177 $\pm$ 0.451  & 0.096 $\pm$ 0.001 & 0.055 $\pm$ 0.001 & 1.0 & 1.0 &  31.04 $\pm$ 8.76  & 22.91 $\pm$ 5.41  \\ 
G016.86$-$02.15         & 17.60  & 5.97  $\pm$ 0.47 & 5.396 $\pm$ 1.089  & 0.244 $\pm$ 0.002 & 0.110 $\pm$ 0.001 & 1.1 & 1.1 &  22.62 $\pm$ 4.36  & 24.20 $\pm$ 4.66  \\ 
G017.02$-$02.40         & 19.91  & 6.40  $\pm$ 0.36 & 4.005 $\pm$ 0.805  & 0.191 $\pm$ 0.002 & 0.078 $\pm$ 0.001 & 1.1 & 1.0 &  20.71 $\pm$ 3.98  & 23.03 $\pm$ 4.42  \\ 
G017.63$+$00.15         & 22.41  & 6.77  $\pm$ 0.04 & 3.027 $\pm$ 0.606  & 0.126 $\pm$ 0.001 & 0.057 $\pm$ 0.001 & 1.1 & 1.0 &  18.19 $\pm$ 3.84  & 22.05 $\pm$ 4.91  \\ 
G018.34$+$01.76         & 33.53  & 6.31  $\pm$ 0.07 & 2.168 $\pm$ 0.436  & 0.109 $\pm$ 0.001 & 0.043 $\pm$ 0.000 & 1.1 & 1.0 &  18.72 $\pm$ 3.60  & 21.29 $\pm$ 4.08  \\ 
G019.00$-$00.02         & 59.71  & 4.55  $\pm$ 0.84 & 2.031 $\pm$ 0.417  & 0.117 $\pm$ 0.001 & 0.048 $\pm$ 0.000 & 1.1 & 1.0 &  21.11 $\pm$ 5.23  &     $\cdots$      \\ 
G019.36$-$00.03         & 26.40  & 5.58  $\pm$ 0.49 & 7.251 $\pm$ 1.470  & 0.381 $\pm$ 0.004 & 0.153 $\pm$ 0.002 & 1.2 & 1.1 &  17.51 $\pm$ 3.39  & 20.09 $\pm$ 3.89  \\ 
G022.35$+$00.06         & 84.17  & 4.49  $\pm$ 1.46 & 3.948 $\pm$ 0.811  & 0.200 $\pm$ 0.002 & 0.094 $\pm$ 0.001 & 1.1 & 1.0 &  13.31 $\pm$ 3.31  & 17.13 $\pm$ 4.21  \\ 
G023.20$-$00.37         & 77.61  & 4.64  $\pm$ 0.43 & 6.823 $\pm$ 1.399  & 0.341 $\pm$ 0.003 & 0.159 $\pm$ 0.002 & 1.2 & 1.1 &  22.17 $\pm$ 4.73  & 18.57 $\pm$ 3.76  \\ 
G023.38$+$00.18         & 75.57  & 4.22  $\pm$ 0.37 & 3.793 $\pm$ 0.783  & 0.148 $\pm$ 0.001 & 0.093 $\pm$ 0.001 & 1.1 & 1.0 &  18.72 $\pm$ 4.97  &     $\cdots$      \\ 
G023.43$-$00.18         & 102.10 & 3.63  $\pm$ 0.49 & 5.077 $\pm$ 1.057  & 0.284 $\pm$ 0.003 & 0.133 $\pm$ 0.001 & 1.1 & 1.1 &  17.21 $\pm$ 3.43  & 18.44 $\pm$ 3.68  \\ 
G024.63$-$00.32         & 42.69  & 4.75  $\pm$ 0.53 & 4.346 $\pm$ 0.890  & 0.223 $\pm$ 0.002 & 0.100 $\pm$ 0.001 & 1.1 & 1.1 &  25.42 $\pm$ 5.86  &     $\cdots$      \\ 
G024.78$+$00.08         & 110.70 & 3.51  $\pm$ 0.15 & 14.485 $\pm$ 3.024 & 0.743 $\pm$ 0.007 & 0.386 $\pm$ 0.004 & 1.4 & 1.2 &  17.50 $\pm$ 3.48  & 20.84 $\pm$ 4.14  \\ 
G024.85$+$00.08         & 109.00 & 3.85  $\pm$ 0.23 & 5.589 $\pm$ 1.160  & 0.301 $\pm$ 0.003 & 0.143 $\pm$ 0.001 & 1.2 & 1.1 &  17.84 $\pm$ 3.76  & 17.87 $\pm$ 3.70  \\ 
G028.14$-$00.00         & 98.72  & 3.96  $\pm$ 0.21 & 3.678 $\pm$ 0.762  & 0.315 $\pm$ 0.003 & 0.093 $\pm$ 0.001 & 1.2 & 1.0 &  13.29 $\pm$ 3.64  & 14.86 $\pm$ 3.97  \\ 
G028.30$-$00.38         & 85.55  & 4.71  $\pm$ 0.26 & 4.379 $\pm$ 0.897  & 0.185 $\pm$ 0.002 & 0.101 $\pm$ 0.001 & 1.1 & 1.1 &  20.14 $\pm$ 4.22  & 21.64 $\pm$ 4.55  \\ 
G028.39$+$00.08         & 78.01  & 4.83  $\pm$ 0.17 & 8.785 $\pm$ 1.797  & 0.320 $\pm$ 0.003 & 0.201 $\pm$ 0.002 & 1.2 & 1.1 &  22.33 $\pm$ 4.37  & 21.50 $\pm$ 4.19  \\ 
G028.83$-$00.25         & 87.19  & 4.50  $\pm$ 0.48 & 7.885 $\pm$ 1.620  & 0.420 $\pm$ 0.004 & 0.187 $\pm$ 0.002 & 1.2 & 1.1 &  17.23 $\pm$ 3.37  & 19.00 $\pm$ 3.72  \\ 
G030.19$-$00.16         & 103.10 & 4.74  $\pm$ 0.11 & 3.792 $\pm$ 0.777  & 0.199 $\pm$ 0.002 & 0.087 $\pm$ 0.001 & 1.1 & 1.0 &  13.89 $\pm$ 3.24  & 17.04 $\pm$ 3.72  \\ 
G030.22$-$00.18         & 103.90 & 5.43  $\pm$ 0.26 & 2.214 $\pm$ 0.449  & 0.135 $\pm$ 0.001 & 0.047 $\pm$ 0.000 & 1.1 & 1.0 &  13.01 $\pm$ 3.94  & 32.85 $\pm$ 8.06  \\ 
G030.41$-$00.23         & 105.10 & 5.17  $\pm$ 0.20 & 2.345 $\pm$ 0.478  & 0.127 $\pm$ 0.001 & 0.052 $\pm$ 0.001 & 1.1 & 1.0 &  23.09 $\pm$ 5.08  & 23.79 $\pm$ 5.42  \\ 
G030.70$-$00.06         & 89.94  & 4.20  $\pm$ 0.10 & 11.017 $\pm$ 2.274 & 0.495 $\pm$ 0.005 & 0.270 $\pm$ 0.003 & 1.3 & 1.1 &  21.56 $\pm$ 4.24  & 22.96 $\pm$ 4.51  \\ 
G030.74$-$00.04         & 91.83  & 5.76  $\pm$ 0.36 & 9.418 $\pm$ 1.905  & 0.437 $\pm$ 0.004 & 0.195 $\pm$ 0.002 & 1.2 & 1.1 &  19.79 $\pm$ 3.82  & 22.80 $\pm$ 4.39  \\ 
G030.78$+$00.20         & 81.94  & 4.19  $\pm$ 0.05 & 6.244 $\pm$ 1.289  & 0.342 $\pm$ 0.003 & 0.153 $\pm$ 0.002 & 1.2 & 1.1 &  15.01 $\pm$ 3.26  & 18.83 $\pm$ 3.91  \\ 
G030.81$-$00.05         & 98.90  & 5.73  $\pm$ 0.24 & 9.272 $\pm$ 1.876  & 0.337 $\pm$ 0.003 & 0.193 $\pm$ 0.002 & 1.2 & 1.1 &  24.57 $\pm$ 4.74  & 25.88 $\pm$ 4.98  \\ 
G031.24$-$00.11         & 21.08  & 7.48  $\pm$ 2.00 & 3.306 $\pm$ 0.658  & 0.135 $\pm$ 0.001 & 0.059 $\pm$ 0.001 & 1.1 & 1.0 &  24.86 $\pm$ 5.18  & 22.93 $\pm$ 4.53  \\ 
G032.74$-$00.07         & 37.21  & 4.55  $\pm$ 0.23 & 5.966 $\pm$ 1.225  & 0.254 $\pm$ 0.003 & 0.140 $\pm$ 0.001 & 1.1 & 1.1 &  19.81 $\pm$ 3.89  & 22.14 $\pm$ 4.33  \\ 
G032.79$+$00.19         & 14.15  & 5.26  $\pm$ 1.57 & 3.793 $\pm$ 0.772  & 0.192 $\pm$ 0.002 & 0.083 $\pm$ 0.001 & 1.1 & 1.0 &  19.77 $\pm$ 3.83  & 21.92 $\pm$ 4.25  \\ 
G034.41$+$00.23         & 57.73  & 5.99  $\pm$ 0.06 & 4.573 $\pm$ 0.923  & 0.211 $\pm$ 0.002 & 0.093 $\pm$ 0.001 & 1.1 & 1.0 &  21.42 $\pm$ 4.13  & 24.13 $\pm$ 4.64  \\ 
G034.79$-$01.38         & 45.95  & 6.21  $\pm$ 0.09 & 13.430 $\pm$ 2.704 & 0.625 $\pm$ 0.006 & 0.267 $\pm$ 0.003 & 1.3 & 1.1 &  18.70 $\pm$ 3.60  & 22.32 $\pm$ 4.30  \\ 
G035.79$-$00.17         & 61.48  & 5.27  $\pm$ 0.43 & 4.295 $\pm$ 0.874  & 0.227 $\pm$ 0.002 & 0.094 $\pm$ 0.001 & 1.1 & 1.0 &  18.58 $\pm$ 4.89  & 23.95 $\pm$ 5.17  \\ 
G036.11$+$00.55         & 76.15  & 5.45  $\pm$ 0.43 & 9.082 $\pm$ 1.844  & 0.416 $\pm$ 0.004 & 0.194 $\pm$ 0.002 & 1.2 & 1.1 &  16.78 $\pm$ 4.34  & 23.71 $\pm$ 5.64  \\ 
G037.42$+$01.51         & 43.87  & 6.78  $\pm$ 0.05 & 2.584 $\pm$ 0.517  & 0.118 $\pm$ 0.001 & 0.049 $\pm$ 0.000 & 1.1 & 1.0 &  21.29 $\pm$ 4.06  & 23.33 $\pm$ 4.45  \\ 
G038.11$-$00.22         & 83.12  & 5.55  $\pm$ 0.25 & 5.925 $\pm$ 1.201  & 0.277 $\pm$ 0.003 & 0.125 $\pm$ 0.001 & 1.1 & 1.1 &  21.63 $\pm$ 5.23  & 21.60 $\pm$ 5.00  \\ 
G040.28$-$00.21         & 73.65  & 6.02  $\pm$ 0.10 & 6.889 $\pm$ 1.390  & 0.348 $\pm$ 0.003 & 0.139 $\pm$ 0.001 & 1.2 & 1.1 &  19.54 $\pm$ 4.06  & 21.71 $\pm$ 4.32  \\ 
G040.42$+$00.70         & 12.50  & 8.46  $\pm$ 1.67 & 2.892 $\pm$ 0.571  & 0.194 $\pm$ 0.196 & 0.047 $\pm$ 0.000 & 1.1 & 1.0 &  16.43 $\pm$ 6.11  & 28.68 $\pm$ 6.15  \\ 
G040.62$-$00.13         & 32.84  & 8.24  $\pm$ 2.50 & 2.458 $\pm$ 0.486  & 0.108 $\pm$ 0.001 & 0.041 $\pm$ 0.000 & 1.1 & 1.0 &  25.95 $\pm$ 5.94  & 25.00 $\pm$ 6.17  \\ 
G043.03$-$00.45         & 57.54  & 5.84  $\pm$ 0.33 & 5.524 $\pm$ 1.116  & 0.229 $\pm$ 0.002 & 0.114 $\pm$ 0.001 & 1.1 & 1.1 &  22.25 $\pm$ 4.63  & 22.26 $\pm$ 4.50  \\ 
G045.45$+$00.06         & 58.08  & 6.41  $\pm$ 0.50 & 4.570 $\pm$ 0.918  & 0.211 $\pm$ 0.002 & 0.089 $\pm$ 0.001 & 1.1 & 1.0 &  24.64 $\pm$ 4.99  & 25.31 $\pm$ 5.02  \\ 
G045.49$+$00.12         & 60.59  & 5.96  $\pm$ 0.24 & 5.985 $\pm$ 1.208  & 0.174 $\pm$ 0.002 & 0.122 $\pm$ 0.001 & 1.1 & 1.1 &  14.53 $\pm$ 3.84  &     $\cdots$      \\ 
G045.80$-$00.35         & 59.12  & 6.08  $\pm$ 0.32 & 6.549 $\pm$ 1.320  & 0.300 $\pm$ 0.003 & 0.132 $\pm$ 0.001 & 1.2 & 1.1 &  16.95 $\pm$ 3.98  & 22.31 $\pm$ 4.84  \\ 
G048.99$-$00.29         & 68.01  & 6.18  $\pm$ 0.02 & 2.061 $\pm$ 0.415  & 0.106 $\pm$ 0.001 & 0.041 $\pm$ 0.000 & 1.1 & 1.0 &  20.75 $\pm$ 4.21  & 21.64 $\pm$ 4.32  \\ 
G049.59$-$00.24         & 57.06  & 6.27  $\pm$ 0.02 & 2.366 $\pm$ 0.476  & 0.157 $\pm$ 0.158 & 0.047 $\pm$ 0.000 & 1.1 & 1.0 &  13.99 $\pm$ 5.57  & 18.91 $\pm$ 5.12  \\ 
W51-IRS2                & 61.09  & 6.22  $\pm$ 0.06 & 2.989 $\pm$ 0.602  & 0.141 $\pm$ 0.001 & 0.059 $\pm$ 0.001 & 1.1 & 1.0 &  21.84 $\pm$ 4.18  & 23.81 $\pm$ 4.56  \\ 
G054.10$-$00.08         & 38.45  & 6.64  $\pm$ 0.04 & 4.402 $\pm$ 0.883  & 0.198 $\pm$ 0.002 & 0.084 $\pm$ 0.001 & 1.1 & 1.0 &  19.72 $\pm$ 4.24  & 21.14 $\pm$ 4.46  \\ 
G058.77$+$00.64         & 32.36  & 7.05  $\pm$ 0.06 & 2.964 $\pm$ 0.592  & 0.150 $\pm$ 0.002 & 0.055 $\pm$ 0.001 & 1.1 & 1.0 &  22.44 $\pm$ 5.12  & 21.72 $\pm$ 4.74  \\ 
G059.83$+$00.67         & 34.70  & 7.07  $\pm$ 0.00 & 3.534 $\pm$ 0.706  & 0.176 $\pm$ 0.002 & 0.065 $\pm$ 0.001 & 1.1 & 1.0 &  18.31 $\pm$ 4.32  & 22.08 $\pm$ 4.58  \\ 
G060.57$-$00.18         & 4.84   & 8.29  $\pm$ 0.52 & 4.541 $\pm$ 0.898  & 0.140 $\pm$ 0.001 & 0.075 $\pm$ 0.001 & 1.1 & 1.0 &  23.60 $\pm$ 9.45  & 42.80 $\pm$ 12.23 \\ 
G071.31$+$00.82         & 9.00   & 8.02  $\pm$ 0.16 & 4.412 $\pm$ 0.874  & 0.195 $\pm$ 0.002 & 0.075 $\pm$ 0.001 & 1.1 & 1.0 &  17.34 $\pm$ 3.80  & 22.69 $\pm$ 4.66  \\ 
G071.52$-$00.38         & 10.65  & 7.82  $\pm$ 0.04 & 2.923 $\pm$ 0.580  & 0.117 $\pm$ 0.001 & 0.050 $\pm$ 0.001 & 1.1 & 1.0 &  14.12 $\pm$ 4.52  &     $\cdots$      \\ 
G073.65$+$00.19         & -73.62 & 13.54 $\pm$ 2.90 & 3.881 $\pm$ 0.747  & 0.141 $\pm$ 0.001 & 0.045 $\pm$ 0.000 & 1.1 & 1.0 &  28.94 $\pm$ 6.82  & 31.38 $\pm$ 6.33  \\ 
G075.29$+$01.32         & -56.64 & 10.69 $\pm$ 0.58 & 3.360 $\pm$ 0.655  & 0.143 $\pm$ 0.001 & 0.047 $\pm$ 0.000 & 1.1 & 1.0 &  25.97 $\pm$ 5.10  & 23.37 $\pm$ 4.50  \\ 
DR21                    & -2.50  & 8.10  $\pm$ 0.00 & 6.458 $\pm$ 1.278  & 0.285 $\pm$ 0.003 & 0.108 $\pm$ 0.001 & 1.1 & 1.1 &  21.92 $\pm$ 4.12  & 24.85 $\pm$ 4.67  \\ 
G090.92$+$01.48         & -71.92 & 10.13 $\pm$ 0.63 & 3.569 $\pm$ 0.698  & 0.139 $\pm$ 0.001 & 0.052 $\pm$ 0.001 & 1.1 & 1.0 &  22.08 $\pm$ 4.36  & 26.30 $\pm$ 5.12  \\ 
G097.53$+$03.18         & -71.18 & 11.81 $\pm$ 0.70 & 4.859 $\pm$ 0.942  & 0.181 $\pm$ 0.002 & 0.063 $\pm$ 0.001 & 1.1 & 1.0 &  27.98 $\pm$ 5.21  & 28.27 $\pm$ 5.24  \\ 
G108.20$+$00.58         & -50.70 & 10.43 $\pm$ 0.48 & 1.816 $\pm$ 0.355  & 0.109 $\pm$ 0.110 & 0.026 $\pm$ 0.000 & 1.1 & 1.0 &  21.62 $\pm$ 5.66  & 21.84 $\pm$ 6.25  \\ 
G109.87$+$02.11         & -10.88 & 8.49  $\pm$ 0.01 & 2.944 $\pm$ 0.582  & 0.141 $\pm$ 0.001 & 0.048 $\pm$ 0.000 & 1.1 & 1.0 &  20.98 $\pm$ 3.97  & 22.24 $\pm$ 4.24  \\ 
NGC7538                 & -57.12 & 9.47  $\pm$ 0.07 & 3.293 $\pm$ 0.646  & 0.136 $\pm$ 0.001 & 0.050 $\pm$ 0.000 & 1.1 & 1.0 &  23.92 $\pm$ 4.46  & 25.81 $\pm$ 4.81  \\ 
\hline
 \end{longtable}
\tablefoot{ Velocities were obtained from measurements of C$^{34}$S, see Table \ref{fitting_all}. The $^{32}$S/$^{34}$S isotope ratios from the $J$ = 2-1 transition are corrected for the optical depth effect and the ones in the 3-2 line without corrections of opacity.  }
\end{center}

==> newTables/1ratiosTable13c34s-all.tex <==
\begin{table*}[h]
\caption{Isotope ratios derived with the $J$ = 2-1 transitions of C$^{34}$S, $^{13}$CS, and $^{13}$C$^{34}$S.}
\centering
\small
\begin{tabular}{lcc|ccc|cc|cc}
\hline\hline
%\tablenum{2}
Source &  $V_{\rm LSR}$ & $R_{GC}$  &   \multicolumn{3}{c}{Optical depth}  &   \multicolumn{2}{c}{Corrections for} &  $^{12}$C/$^{13}$C  &  $^{32}$S/$^{34}$S  \\
  &                &         &     &           &           &  \multicolumn{2}{c}{optical depth} &   &    \\
  &  (km s$^{-1}$) & (kpc)   &  CS & C$^{34}$S & $^{13}$CS &  $f_1$  &  $f_2$ &   &    \\
\hline
\label{table_13c34sresults}
W3OH                    & -46.96 &  9.64 $\pm$ 0.03   & 8.289 $\pm$ 0.083 & 0.292 $\pm$ 0.003 & 0.127 $\pm$ 0.001 &  1.2  &  1.1  &  75.30 $\pm$ 4.27  &    29.80 $\pm$ 1.68 \\
Orion-KL                &   8.17 &  8.54 $\pm$ 0.00   & 3.722 $\pm$ 0.037 & 0.180 $\pm$ 0.002 & 0.074 $\pm$ 0.001 &  1.1  &  1.0  &  54.89 $\pm$ 12.90 &    21.24 $\pm$ 4.67 \\
G359.61$-$00.24         &  19.33 &  5.51 $\pm$ 0.15   & 3.531 $\pm$ 0.035 & 0.204 $\pm$ 0.002 & 0.089 $\pm$ 0.001 &  1.1  &  1.0  &  43.85 $\pm$ 11.95 &    17.31 $\pm$ 4.79 \\
$+$50~km~s$^{-1}$~cloud &  46.79 &  0.02 $\pm$ 0.04   & 4.278 $\pm$ 0.043 & 0.192 $\pm$ 0.002 & 0.151 $\pm$ 0.002 &  1.1  &  1.1  &  31.22 $\pm$ 2.06  &    21.71 $\pm$ 1.40 \\
SgrB2                   &  53.18 &  0.55 $\pm$ 0.05   & 1.290 $\pm$ 0.013 & 0.140 $\pm$ 0.001 & 0.113 $\pm$ 0.001 &  1.1  &  1.1  &  12.18 $\pm$ 0.73  &    9.77  $\pm$ 0.58 \\
SgrB2                   &  66.54 &  0.44 $\pm$ 0.70   & 8.119 $\pm$ 0.081 & 0.523 $\pm$ 0.005 & 0.341 $\pm$ 0.003 &  1.3  &  1.2  &  30.62 $\pm$ 2.04  &    18.99 $\pm$ 1.31 \\
SgrB2                   &  83.38 &  0.41 $\pm$ 0.02   & 2.417 $\pm$ 0.024 & 0.097 $\pm$ 0.001 & 0.077 $\pm$ 0.001 &  1.0  &  1.0  &  32.90 $\pm$ 5.65  &    26.24 $\pm$ 4.49 \\
G006.79$-$00.25         &  20.87 &  4.75 $\pm$ 0.25   & 8.789 $\pm$ 0.088 & 0.484 $\pm$ 0.005 & 0.242 $\pm$ 0.002 &  1.3  &  1.1  &  45.82 $\pm$ 8.39  &    19.46 $\pm$ 3.63 \\
G010.32$-$00.15         &  11.99 &  5.34 $\pm$ 0.29   & 5.039 $\pm$ 0.050 & 0.237 $\pm$ 0.002 & 0.111 $\pm$ 0.001 &  1.1  &  1.1  &  50.95 $\pm$ 11.58 &    21.55 $\pm$ 5.05 \\
G019.36$-$00.03         &  26.40 &  5.58 $\pm$ 0.49   & 6.789 $\pm$ 0.068 & 0.332 $\pm$ 0.003 & 0.141 $\pm$ 0.001 &  1.2  &  1.1  &  56.41 $\pm$ 14.37 &    21.19 $\pm$ 5.53 \\
G024.78$+$00.08         & 110.72 &  3.51 $\pm$ 0.15   & 8.038 $\pm$ 0.080 & 0.554 $\pm$ 0.006 & 0.322 $\pm$ 0.003 &  1.3  &  1.2  &  32.56 $\pm$ 4.25  &    16.08 $\pm$ 2.12 \\
G028.39$+$00.08         &  78.01 &  4.83 $\pm$ 0.17   & 8.705 $\pm$ 0.087 & 0.443 $\pm$ 0.004 & 0.291 $\pm$ 0.003 &  1.2  &  1.2  &  37.04 $\pm$ 10.05 &    18.74 $\pm$ 5.12 \\
G028.83$-$00.25         &  87.19 &  4.50 $\pm$ 0.48   & 7.283 $\pm$ 0.073 & 0.388 $\pm$ 0.004 & 0.183 $\pm$ 0.002 &  1.2  &  1.1  &  47.93 $\pm$ 10.00 &    19.73 $\pm$ 4.16 \\
G030.70$-$00.06         &  89.94 &  4.20 $\pm$ 0.10   & 7.088 $\pm$ 0.071 & 0.448 $\pm$ 0.004 & 0.263 $\pm$ 0.003 &  1.2  &  1.1  &  33.39 $\pm$ 2.77  &    18.07 $\pm$ 1.52 \\
G030.74$-$00.04         &  91.82 &  5.76 $\pm$ 0.36   & 5.924 $\pm$ 0.059 & 0.404 $\pm$ 0.004 & 0.191 $\pm$ 0.002 &  1.2  &  1.1  &  37.63 $\pm$ 10.87 &    15.61 $\pm$ 4.59 \\
G030.81$-$00.05         &  98.89 &  5.73 $\pm$ 0.24   & 4.691 $\pm$ 0.047 & 0.306 $\pm$ 0.003 & 0.187 $\pm$ 0.002 &  1.2  &  1.1  &  29.07 $\pm$ 2.99  &    14.97 $\pm$ 1.44 \\
W51-IRS2                &  61.07 &  6.22 $\pm$ 0.06   & 1.883 $\pm$ 0.019 & 0.119 $\pm$ 0.001 & 0.052 $\pm$ 0.001 &  1.1  &  1.0  &  38.26 $\pm$ 4.35  &    16.70 $\pm$ 1.92 \\
DR21                    &  -2.49 &  8.10 $\pm$ 0.00   & 7.079 $\pm$ 0.071 & 0.270 $\pm$ 0.003 & 0.106 $\pm$ 0.001 &  1.1  &  1.1  &  76.22 $\pm$ 7.57  &    27.48 $\pm$ 2.84 \\
NGC7538                 & -57.12 &  9.47 $\pm$ 0.07   & 3.433 $\pm$ 0.034 & 0.131 $\pm$ 0.001 & 0.050 $\pm$ 0.001 &  1.1  &  1.0  &  73.19 $\pm$ 12.54 &    26.72 $\pm$ 4.57 \\
\hline
\end{tabular}
\tablefoot{ Velocities were obtained from measurements of C$^{34}$S, see Table \ref{fitting_all} in Appendix \ref{appendix_table}.}
\end{table*}

==> newTables/32s-33sTable-corrected.tex <==
\begin{table*}[h]
\centering
\caption{\label{table_3233}  $^{32}$S/$^{33}$S isotope ratios}
\begin{tabular}{lccc}
\hline\hline
Source &  $R_{GC}$  &   \multicolumn{2}{c}{$^{32}$S/$^{33}$S}  \\
       &  (kpc)     &  $J$ = 2-1    &     $J$ = 3-2       \\
\hline
WB89-380 & 14.19 $\pm$ 0.92                & 90.74  $\pm$ 19.53  &   83.93  $\pm$ 17.90  \\
WB89-391 & 14.28 $\pm$ 0.94                & 127.07 $\pm$ 40.26  &   65.46  $\pm$ 14.69  \\
W3OH & 9.64 $\pm$ 0.03                     & 105.49 $\pm$ 7.26   &   74.20  $\pm$ 4.35   \\
Orion-KL & 8.54 $\pm$ 0.00                 & 74.50  $\pm$ 16.85  &   69.12  $\pm$ 13.51  \\
$+$20 km~s$^{-1}$ cloud & 0.03 $\pm$ 0.03  & 82.63  $\pm$ 18.20  &   78.98  $\pm$ 17.86  \\
G359.61$-$00.24 & 5.51 $\pm$ 0.15          & 75.75  $\pm$ 14.99  &   71.69  $\pm$ 16.86  \\
$+$50 km~s$^{-1}$ cloud & 0.02 $\pm$ 0.04  & 76.49  $\pm$ 16.96  &   66.68  $\pm$ 14.92  \\
G000.31$-$00.20 & 5.25 $\pm$ 0.36          & 55.61  $\pm$ 14.84  &   $\cdots$           \\
SgrB2 & 0.44 $\pm$ 0.70                    & 42.98  $\pm$ 9.62   &   35.66  $\pm$ 7.84   \\
SgrD & 0.45 $\pm$ 0.07                     & 77.48  $\pm$ 20.88  &   50.61  $\pm$ 13.66  \\
G006.79$-$00.25 & 4.75 $\pm$ 0.25          & 86.65  $\pm$ 17.01  &   70.08  $\pm$ 13.79  \\
G007.47$+$00.05 & 12.35 $\pm$ 2.49         & 107.98 $\pm$ 30.91  &   $\cdots$           \\
G010.32$-$00.15 & 5.34 $\pm$ 0.29          & 88.27  $\pm$ 17.82  &   79.56  $\pm$ 15.99  \\
G010.62$-$00.33 & 4.26 $\pm$ 0.21          & 106.56 $\pm$ 33.99  &   $\cdots$           \\
G011.10$-$00.11 & 5.49 $\pm$ 0.56          & 72.13  $\pm$ 29.12  &   $\cdots$           \\
G016.86$-$02.15 & 5.97 $\pm$ 0.47          & 86.63  $\pm$ 17.00  &   76.23  $\pm$ 15.01  \\
G017.02$-$02.40 & 6.40 $\pm$ 0.36          & 100.03 $\pm$ 20.54  &   86.36  $\pm$ 17.47  \\
G017.63$+$00.15 & 6.77 $\pm$ 0.04          & 73.12  $\pm$ 23.04  &   $\cdots$           \\
G018.34$+$01.76 & 6.31 $\pm$ 0.07          & 92.66  $\pm$ 18.57  &   86.44  $\pm$ 16.87  \\
G019.36$-$00.03 & 5.58 $\pm$ 0.49          & 94.55  $\pm$ 18.78  &   80.16  $\pm$ 15.89  \\
G023.43$-$00.18 & 3.63 $\pm$ 0.49          & 72.63  $\pm$ 16.26  &   80.58  $\pm$ 16.63  \\
G024.78$+$00.08 & 3.51 $\pm$ 0.15          & 70.88  $\pm$ 14.22  &   55.64  $\pm$ 11.12  \\
G024.85$+$00.08 & 3.85 $\pm$ 0.23          & 134.87 $\pm$ 43.15  &   48.25  $\pm$ 11.88  \\
G028.30$-$00.38 & 4.71 $\pm$ 0.26          & $\cdots$            &   76.82  $\pm$ 20.06  \\
G028.39$+$00.08 & 4.83 $\pm$ 0.17          & 85.30  $\pm$ 17.17  &   76.11  $\pm$ 15.02  \\
G028.83$-$00.25 & 4.50 $\pm$ 0.48          & 78.57  $\pm$ 15.87  &   80.37  $\pm$ 15.83  \\
G030.70$-$00.06 & 4.20 $\pm$ 0.10          & 76.54  $\pm$ 15.18  &   62.68  $\pm$ 12.57  \\
G030.74$-$00.04 & 5.76 $\pm$ 0.36          & 86.28  $\pm$ 17.07  &   72.73  $\pm$ 14.12  \\
G030.78$+$00.20 & 4.19 $\pm$ 0.05          & $\cdots$            &   72.50  $\pm$ 17.46  \\
G030.81$-$00.05 & 5.73 $\pm$ 0.24          & 88.21  $\pm$ 17.23  &   72.72  $\pm$ 14.52  \\
G031.24$-$00.11 & 7.48 $\pm$ 2.00          & $\cdots$            &   90.57  $\pm$ 21.01  \\
G032.74$-$00.07 & 4.55 $\pm$ 0.23          & 75.67  $\pm$ 14.99  &   68.63  $\pm$ 13.88  \\
G032.79$+$00.19 & 5.26 $\pm$ 1.57          & 79.87  $\pm$ 16.07  &   76.72  $\pm$ 14.93  \\
G034.41$+$00.23 & 5.99 $\pm$ 0.06          & 80.54  $\pm$ 15.82  &   72.63  $\pm$ 14.63  \\
G034.79$-$01.38 & 6.21 $\pm$ 0.09          & 103.60 $\pm$ 22.03  &   82.58  $\pm$ 16.21  \\
G036.11$+$00.55 & 5.45 $\pm$ 0.43          & 39.43  $\pm$ 13.64  &   $\cdots$           \\
G037.42$+$01.51 & 6.78 $\pm$ 0.05          & 110.92 $\pm$ 21.76  &   76.06  $\pm$ 17.77  \\
G040.28$-$00.21 & 6.02 $\pm$ 0.10          & 110.40 $\pm$ 31.44  &   71.86  $\pm$ 17.32  \\
G045.45$+$00.06 & 6.41 $\pm$ 0.50          & 83.04  $\pm$ 21.44  &   76.44  $\pm$ 16.33  \\
G048.99$-$00.29 & 6.18 $\pm$ 0.02          & 107.90 $\pm$ 27.60  &   87.21  $\pm$ 20.50  \\
W51-IRS2 & 6.22 $\pm$ 0.06                 & 74.69  $\pm$ 14.46  &   66.43  $\pm$ 12.72  \\
G071.31$+$00.82 & 8.02 $\pm$ 0.16          & 95.37  $\pm$ 31.90  &   106.87 $\pm$ 30.60  \\
G073.65$+$00.19 & 13.54 $\pm$ 2.90         & 102.16 $\pm$ 32.61  &   128.66 $\pm$ 31.17  \\
G075.29$+$01.32 & 10.69 $\pm$ 0.58         & 122.06 $\pm$ 29.02  &   92.08  $\pm$ 19.53  \\
DR21 & 8.10 $\pm$ 0.00                     & 86.80  $\pm$ 16.37  &   80.51  $\pm$ 15.38  \\
G090.92$+$01.48 & 10.13 $\pm$ 0.63         & 87.88  $\pm$ 19.68  &   95.73  $\pm$ 20.14  \\
G097.53$+$03.18 & 11.81 $\pm$ 0.70         & 74.99  $\pm$ 14.50  &   87.92  $\pm$ 16.65  \\
G109.87$+$02.11 & 8.49 $\pm$ 0.01          & 94.41  $\pm$ 18.40  &   98.52  $\pm$ 23.17  \\
NGC7538 & 9.47 $\pm$ 0.07                  & 104.53 $\pm$ 19.54  &   $\cdots$           \\
\hline
\end{tabular}
\tablefoot{The $^{32}$S/$^{33}$S isotope ratios from the $J$ = 2-1 transition are corrected for the line saturation effects, while the ones in the 3-2 line are not corrected due to the missing main isotopic species.}
\end{table*}

==> newTables/c34-c33sTable-corrected.tex <==
\begin{center}
\begin{longtable}{lc|cccc|cccc}
\caption{\label{table_3433}Corrected $^{34}$S/$^{33}$S isotope ratios.}\\
\hline\hline
Source &  $R_{GC}$  &   \multicolumn{4}{c}{$J$ = 2-1} &  \multicolumn{4}{c}{$J$ = 3-2} \\
       &          & FWHM  & C$^{34}$S/C$^{33}$S & $f_{21HFS}$ & $^{34}$S/$^{33}$S &  FWHM & C$^{34}$S/C$^{33}$S & $f_{32HFS}$ & $^{34}$S/$^{33}$S  \\
       &  (kpc)     &   (km s$^{-1}$)   &                     &                               &              &    (km s$^{-1}$)      &           &            &        \\
\hline
\endfirsthead
\caption{continued.}\\
\hline\hline
Source &  $R_{GC}$  &   \multicolumn{4}{c}{$J$ = 2-1} &  \multicolumn{4}{c}{$J$ = 3-2} \\
       &            & FWHM  & C$^{34}$S/C$^{33}$S & $f21_{HFS}$ & $^{34}$S/$^{33}$S  &  FWHM  & C$^{34}$S/C$^{33}$S & $f32_{HFS}$ & $^{34}$S/$^{33}$S  \\
       &  (kpc)     &   (km s$^{-1}$)   &                     &                               &                   &           (km s$^{-1}$)        &           &        &            \\
\hline
\endhead
\hline
\endfoot
WB89-380                & 14.19 $\pm$ 0.92 & 3.60  & 5.70 $\pm$ 0.58 & 0.70 & 4.28 $\pm$ 0.44  & 3.87  & 3.70 $\pm$ 0.37 & 0.91 & 3.36 $\pm$ 0.34  \\ 
WB89-391                & 14.28 $\pm$ 0.94 & 1.03  & 6.75 $\pm$ 1.71 & 0.69 & 5.21 $\pm$ 1.32  & 2.19  & 3.67 $\pm$ 0.42 & 0.85 & 3.12 $\pm$ 0.36  \\ 
W3OH                    & 9.64 $\pm$ 0.03  & 4.41  & 3.04 $\pm$ 0.12 & 1.00 & 3.54 $\pm$ 0.14  & 6.14  & 2.59 $\pm$ 0.04 & 0.96 & 2.49 $\pm$ 0.04  \\ 
Orion-KL                & 8.54 $\pm$ 0.00  & 4.25  & 2.77 $\pm$ 0.22 & 1.00 & 3.01 $\pm$ 0.24  & 8.33  & 2.74 $\pm$ 0.12 & 0.99 & 2.72 $\pm$ 0.11  \\ 
$+$20~km~s$^{-1}$~cloud & 0.03 $\pm$ 0.03  & 24.78 & 4.89 $\pm$ 0.14 & 1.00 & 5.64 $\pm$ 0.16  & 20.12 & 5.22 $\pm$ 0.30 & 1.00 & 5.22 $\pm$ 0.30  \\ 
G359.61$-$00.24         & 5.51 $\pm$ 0.15  & 3.17  & 3.63 $\pm$ 0.12 & 1.00 & 4.04 $\pm$ 0.13  & 10.44 & 3.33 $\pm$ 0.45 & 0.99 & 3.31 $\pm$ 0.44  \\ 
$+$50~km~s$^{-1}$~cloud & 0.02 $\pm$ 0.04  & 24.29 & 4.80 $\pm$ 0.06 & 1.00 & 5.29 $\pm$ 0.07  & 21.28 & 4.57 $\pm$ 0.15 & 1.00 & 4.57 $\pm$ 0.15  \\ 
G000.31$-$00.20         & 5.25 $\pm$ 0.36  & 3.58  & 4.65 $\pm$ 0.70 & 0.70 & 3.54 $\pm$ 0.53  & $\cdots$ & $\cdots$        & $\cdots$ & $\cdots$   \\ 
SgrB2                   & 0.44 $\pm$ 0.70  & 21.14 & 2.23 $\pm$ 0.10 & 0.99 & 2.46 $\pm$ 0.11  & 21.22 & 2.00 $\pm$ 0.03 & 1.00 & 2.00 $\pm$ 0.03  \\
SgrD                    & 0.45 $\pm$ 0.07  & 2.73  & 7.01 $\pm$ 0.47 & 0.70 & 4.96 $\pm$ 0.33  & 4.00  & 3.56 $\pm$ 0.24 & 0.91 & 3.24 $\pm$ 0.22  \\ 
G006.79$-$00.25         & 4.75 $\pm$ 0.25  & 2.73  & 3.79 $\pm$ 0.08 & 0.98 & 4.79 $\pm$ 0.10  & 3.32  & 3.68 $\pm$ 0.09 & 0.89 & 3.29 $\pm$ 0.08  \\ 
G007.47$+$00.05         & 12.35 $\pm$ 2.49 & 3.12  & 5.41 $\pm$ 0.97 & 0.70 & 4.07 $\pm$ 0.73  & $\cdots$ & $\cdots$        & $\cdots$ & $\cdots$   \\ 
G010.32$-$00.15         & 5.34 $\pm$ 0.29  & 2.66  & 4.16 $\pm$ 0.22 & 0.98 & 4.60 $\pm$ 0.25  & 3.74  & 4.07 $\pm$ 0.21 & 0.90 & 3.68 $\pm$ 0.19  \\ 
G010.62$-$00.33         & 5.49 $\pm$ 0.56  & 2.70  & 6.37 $\pm$ 1.45 & 0.98 & 6.80 $\pm$ 1.54  & $\cdots$ & $\cdots$        & $\cdots$ & $\cdots$   \\ 
G011.10$-$00.11         & 4.26 $\pm$ 0.21  & 1.45  & 5.36 $\pm$ 1.52 & 0.69 & 3.72 $\pm$ 1.05  & $\cdots$ & $\cdots$        & $\cdots$ & $\cdots$   \\ 
G016.86$-$02.15         & 5.97 $\pm$ 0.47  & 3.32  & 3.47 $\pm$ 0.12 & 0.98 & 3.83 $\pm$ 0.14  & 4.33  & 3.42 $\pm$ 0.14 & 0.92 & 3.15 $\pm$ 0.13  \\ 
G017.02$-$02.40         & 6.40 $\pm$ 0.36  & 3.74  & 4.49 $\pm$ 0.33 & 0.98 & 4.83 $\pm$ 0.35  & 4.03  & 4.11 $\pm$ 0.26 & 0.91 & 3.75 $\pm$ 0.24  \\ 
G017.63$+$00.15         & 6.77 $\pm$ 0.04  & 2.74  & 5.41 $\pm$ 1.27 & 0.70 & 4.02 $\pm$ 0.94  & $\cdots$ & $\cdots$        & $\cdots$ & $\cdots$   \\ 
G018.34$+$01.76         & 6.31 $\pm$ 0.07  & 2.30  & 4.79 $\pm$ 0.28 & 0.98 & 4.95 $\pm$ 0.28  & 3.00  & 4.59 $\pm$ 0.16 & 0.88 & 4.06 $\pm$ 0.15  \\ 
G019.36$-$00.03         & 5.58 $\pm$ 0.49  & 3.02  & 4.58 $\pm$ 0.20 & 0.98 & 5.40 $\pm$ 0.24  & 5.09  & 4.25 $\pm$ 0.18 & 0.94 & 3.99 $\pm$ 0.17  \\ 
G023.43$-$00.18         & 3.63 $\pm$ 0.49  & 3.81  & 3.75 $\pm$ 0.38 & 0.98 & 4.22 $\pm$ 0.43  & 5.06  & 4.65 $\pm$ 0.24 & 0.94 & 4.37 $\pm$ 0.23  \\ 
G024.78$+$00.08         & 3.51 $\pm$ 0.15  & 4.29  & 2.86 $\pm$ 0.08 & 1.00 & 4.05 $\pm$ 0.11  & 6.36  & 2.76 $\pm$ 0.06 & 0.96 & 2.67 $\pm$ 0.06  \\ 
G024.85$+$00.08         & 3.85 $\pm$ 0.23  & 1.27  & 9.43 $\pm$ 2.27 & 0.69 & 7.56 $\pm$ 1.82  & 3.20  & 3.03 $\pm$ 0.40 & 0.89 & 2.70 $\pm$ 0.36  \\ 
G028.30$-$00.38         & 4.71 $\pm$ 0.26  & $\cdots$  & $\cdots$        & $\cdots$ & $\cdots$ & 2.68  & 4.05 $\pm$ 0.63 & 0.88 & 3.55 $\pm$ 0.55  \\ 
G028.39$+$00.08         & 4.83 $\pm$ 0.17  & 3.04  & 3.33 $\pm$ 0.15 & 0.98 & 3.82 $\pm$ 0.18  & 4.39  & 3.84 $\pm$ 0.12 & 0.92 & 3.54 $\pm$ 0.11  \\ 
G028.83$-$00.25         & 4.50 $\pm$ 0.48  & 2.27  & 3.80 $\pm$ 0.19 & 0.98 & 4.56 $\pm$ 0.23  & 3.94  & 4.65 $\pm$ 0.10 & 0.91 & 4.23 $\pm$ 0.09  \\ 
G030.70$-$00.06         & 4.20 $\pm$ 0.10  & 4.85  & 2.80 $\pm$ 0.07 & 1.00 & 3.55 $\pm$ 0.09  & 6.29  & 2.84 $\pm$ 0.12 & 0.96 & 2.73 $\pm$ 0.11  \\ 
G030.74$-$00.04         & 5.76 $\pm$ 0.36  & 3.55  & 3.61 $\pm$ 0.15 & 0.98 & 4.36 $\pm$ 0.19  & 4.24  & 3.48 $\pm$ 0.08 & 0.92 & 3.19 $\pm$ 0.08  \\ 
G030.78$+$00.20         & 4.19 $\pm$ 0.05  & $\cdots$  & $\cdots$        & $\cdots$ & $\cdots$ & 4.17  & 4.20 $\pm$ 0.51 & 0.92 & 3.85 $\pm$ 0.47  \\ 
G030.81$-$00.05         & 5.73 $\pm$ 0.24  & 6.15  & 3.05 $\pm$ 0.09 & 1.00 & 3.59 $\pm$ 0.11  & 7.34  & 2.88 $\pm$ 0.15 & 0.98 & 2.81 $\pm$ 0.15  \\ 
G031.24$-$00.11         & 7.48 $\pm$ 2.00  & $\cdots$  & $\cdots$        & $\cdots$ & $\cdots$ & 4.15  & 4.32 $\pm$ 0.52 & 0.92 & 3.95 $\pm$ 0.48  \\ 
G032.74$-$00.07         & 4.55 $\pm$ 0.23  & 4.54  & 3.44 $\pm$ 0.09 & 0.98 & 3.82 $\pm$ 0.10  & 8.07  & 3.15 $\pm$ 0.16 & 0.98 & 3.10 $\pm$ 0.16  \\
G032.79$+$00.19         & 5.26 $\pm$ 1.57  & 4.78  & 3.75 $\pm$ 0.21 & 0.98 & 4.04 $\pm$ 0.22  & 8.17  & 3.56 $\pm$ 0.06 & 0.98 & 3.50 $\pm$ 0.06  \\
G034.41$+$00.23         & 5.99 $\pm$ 0.06  & 4.56  & 3.39 $\pm$ 0.13 & 1.00 & 3.76 $\pm$ 0.14  & 6.28  & 3.13 $\pm$ 0.18 & 0.96 & 3.01 $\pm$ 0.18  \\
G034.79$-$01.38         & 6.21 $\pm$ 0.09  & 2.40  & 4.21 $\pm$ 0.37 & 0.98 & 5.54 $\pm$ 0.50  & 3.34  & 4.14 $\pm$ 0.16 & 0.89 & 3.70 $\pm$ 0.14  \\
G036.11$+$00.55         & 5.45 $\pm$ 0.43  & 2.57  & 2.75 $\pm$ 0.63 & 0.70 & 2.35 $\pm$ 0.54  & $\cdots$ & $\cdots$        & $\cdots$ & $\cdots$   \\ 
G037.42$+$01.51         & 6.78 $\pm$ 0.05  & 3.18  & 5.02 $\pm$ 0.23 & 0.98 & 5.21 $\pm$ 0.24  & 4.78  & 3.50 $\pm$ 0.48 & 0.93 & 3.26 $\pm$ 0.44  \\ 
G040.28$-$00.21         & 6.02 $\pm$ 0.10  & 3.72  & 6.79 $\pm$ 1.33 & 0.70 & 5.65 $\pm$ 1.10  & 6.43  & 3.43 $\pm$ 0.47 & 0.97 & 3.31 $\pm$ 0.45  \\ 
G045.45$+$00.06         & 6.41 $\pm$ 0.50  & 6.08  & 4.07 $\pm$ 0.66 & 0.75 & 3.37 $\pm$ 0.54  & 5.28  & 3.20 $\pm$ 0.25 & 0.94 & 3.02 $\pm$ 0.24  \\ 
G048.99$-$00.29         & 6.18 $\pm$ 0.02  & 3.74  & 7.02 $\pm$ 1.10 & 0.70 & 5.20 $\pm$ 0.81  & 4.78  & 4.32 $\pm$ 0.54 & 0.93 & 4.03 $\pm$ 0.50  \\ 
W51-IRS2                & 6.22 $\pm$ 0.06  & 8.55  & 3.19 $\pm$ 0.09 & 1.00 & 3.42 $\pm$ 0.10  & 8.72  & 2.82 $\pm$ 0.01 & 0.99 & 2.79 $\pm$ 0.01  \\ 
G071.31$+$00.82         & 8.02 $\pm$ 0.16  & 2.25  & 7.18 $\pm$ 1.81 & 0.70 & 5.50 $\pm$ 1.39  & 2.42  & 5.43 $\pm$ 1.08 & 0.87 & 4.71 $\pm$ 0.94  \\ 
G073.65$+$00.19         & 13.54 $\pm$ 2.90 & 2.76  & 4.71 $\pm$ 1.02 & 0.70 & 3.53 $\pm$ 0.76  & 2.88  & 4.65 $\pm$ 0.62 & 0.88 & 4.10 $\pm$ 0.55  \\ 
G075.29$+$01.32         & 10.69 $\pm$ 0.58 & 2.86  & 6.27 $\pm$ 0.85 & 0.70 & 4.70 $\pm$ 0.63  & 2.83  & 4.47 $\pm$ 0.40 & 0.88 & 3.94 $\pm$ 0.35  \\ 
DR21                    & 8.10 $\pm$ 0.00  & 2.71  & 3.45 $\pm$ 0.05 & 1.00 & 3.96 $\pm$ 0.06  & 3.15  & 3.27 $\pm$ 0.11 & 0.99 & 3.24 $\pm$ 0.11  \\ 
G090.92$+$01.48         & 10.13 $\pm$ 0.63 & 3.40  & 5.31 $\pm$ 0.56 & 0.70 & 3.98 $\pm$ 0.42  & 3.79  & 4.02 $\pm$ 0.32 & 0.91 & 3.64 $\pm$ 0.29  \\ 
G097.53$+$03.18         & 11.81 $\pm$ 0.70 & 5.22  & 2.45 $\pm$ 0.13 & 1.00 & 2.68 $\pm$ 0.14  & 5.47  & 3.28 $\pm$ 0.12 & 0.95 & 3.11 $\pm$ 0.12  \\ 
G109.87$+$02.11         & 8.49 $\pm$ 0.01  & 3.19  & 4.28 $\pm$ 0.21 & 0.98 & 4.50 $\pm$ 0.21  & 3.90  & 4.88 $\pm$ 0.67 & 0.91 & 4.43 $\pm$ 0.61  \\ 
NGC7538                 & 9.47 $\pm$ 0.07  & 3.71 & 4.17 $\pm$ 0.07 & 0.98 & 4.37 $\pm$ 0.06  & $\cdots$ & $\cdots$        & $\cdots$ & $\cdots$   \\ 
\hline
 \end{longtable}
\tablefoot{  Full widths to half maximum line widths were obtained from measurements of of C$^{33}$S, see Table \ref{fitting_all}. The $^{34}$S/$^{33}$S isotope ratios from the $J$ = 2-1 transition are corrected for the optical depth effect and the ones in the 3-2 line without corrections for opacity.
}
\end{center}
